A physics-informed neural network framework for modeling obstacle-related equations

Deep learning has been highly successful in some applications. Nevertheless, its use for solving partial differential equations (PDEs) has only been of recent interest with current state-of-the-art machine learning libraries, e.g., TensorFlow or PyTorch. Physics-informed neural networks (PINNs) are an attractive tool for solving partial differential equations based on sparse and noisy data. Here extend PINNs to solve obstacle-related PDEs which present a great computational challenge because they necessitate numerical methods that can yield an accurate approximation of the solution that lies above a given obstacle. The performance of the proposed PINNs is demonstrated in multiple scenarios for linear and nonlinear PDEs subject to regular and irregular obstacles.

==> configurations.tex <==

% 1D:
% phi_1: N_b = 10, N_r = 5000, Layer = 6, nodes = 24, toll = 
% phi_2: N_b = 10, N_r = 5000, Layer = 4, nodes = 24, toll = 
% phi_3: N_b = 10, N_r = 5000, Layer = 4, nodes = 24, toll = 4e-05
% phi_4: N_b = 10, N_r = 5000, Layer = 4, nodes = 24, toll = 2e-6

% phi_5: N_b = 50, N_r = 10000, Layer = 3, nodes = 24, toll = 3e-6
% phi_6: N_b = 50, N_r = 14000, Layer = 4, nodes = 20, toll = 3.7e-04

